Jodes: Efficient Oblivious Join in the Distributed Setting

Trusted execution environment (TEE) has provided an isolated and secure environment for building cloud-based analytic systems, but it still suffers from access pattern leakages caused by side-channel attacks. To better secure the data, computation inside TEE enclave should be made oblivious, which introduces significant overhead and severely slows down the computation. A natural way to speed up is to build the analytic system with multiple servers in the distributed setting. However, this setting raises a new security concern -- the volumes of the transmissions among these servers can leak sensitive information to a network adversary. Existing works have designed specialized algorithms to address this concern, but their supports for equi-join, one of the most important but non-trivial database operators, are either inefficient, limited, or under a weak security assumption. In this paper, we present Jodes, an efficient oblivious join algorithm in the distributed setting. Jodes prevents the leakage on both the network and enclave sides, supports a general equi-join operation, and provides a high security level protection that only publicizes the input sizes and the output size. Meanwhile, it achieves both communication cost and computation cost asymptotically superior to existing algorithms. To demonstrate the practicality of Jodes, we conduct experiments in the distributed setting comprising 16 servers. Empirical results show that Jodes achieves up to a sixfold performance improvement over state-of-the-art join algorithms.

==> main/backup.tex <==
\paragraph{Proof of communication lower bound}
Let $f$ be the join operation, then $\mathcal{A}_1$ is state-of-the-art oblivious join algorithm under the single server model~\cite{10.14778/3407790.3407814} with cost $O(C(N,M))$ where $C(N,M)=(N+M)\log^2 N$. The above definition induces that if $\mathcal{A}_p$ is a perfect load balanced join algorithm, then the computation cost of it is expected to be $O(C(N,M)/p)$.
Based on this, we then provide a lower bound of the communication cost of $\mathcal{A}_1$. First note that the output size of the join in each server is $O(M/p)$, otherwise performing $\mathcal{A}_1$ locally in each server will result in computation cost of $\mathcal{A}_1$ exceeds $O(C(N,M)/p)$. 
% Since the total output size over all the servers is $M$, this suggests that the output size in each server is exactly $\Theta(M/p)$. Note that a server that locally holds $L$ tuples can produce at most $O(L^2)$ join results~\cite{10.1145/3034786.3056110}, hence $L=\Omega(\sqrt{M/p})$. 
$M=\sum_{i=1}^p L_i^2=O(\sqrt{M/p}) \sum_{i=1}^p L_i$, so communication cost $\sum_{i=1}^p L_i=\Omega(\sqrt{Mp})$.

Besides, $L=\Omega(N/p)$ due to holding the input. By Yao's Minimax Principle~\cite{10.1109/SFCS.1977.24}, if we define the input distribution to be a random shuffle of the original one, then only $L/p$ tuples are expected to located in this server without any communication. The overall communication cost is therefore expected to be at least $p(L-L/p)=\Omega(N+\sqrt{Mp})$.

\paragraph{Perfect Load Balanced Join}
The major significance of the distributed model is to distribute the computation cost to $p$ servers for better performance. 
Note that state-of-the-art oblivious join algorithm under the single server model is the one proposed in~\cite{10.14778/3407790.3407814}. Although it claims their cost to be $O(N\log^2 N+M\log M)$, we note that the authors actually missed an extra logarithm term on $M\log M$ which is introduced by the bitonic sort in their Algorithm~5. Therefore, the actual cost of their algorithm is $O(C(N,M))$ where $C(N,M)=(N+M)\log^2 N$, while our algorithm under the distributed model has computation cost $O(C(N,M)/p)$. As a result, we say our algorithm is \textit{perfectly load balanced}.

For any function $f$, let $\mathcal{A}_1$ (\resp $\mathcal{A}_p$) be state-of-the-art algorithm (\ie, with smallest cost) that implements $f$ under the single server model (\resp in the distribute model with $p$ servers), and let $C_1$ (\resp $C_p$) be the computation cost of $\mathcal{A}_1$ (\resp $\mathcal{A}_p$). Then it is guaranteed that $C_1/p\le C_p\le C_1$. The inequality $C_1/p\le C_p$ comes from the fact that one can logically apply $\mathcal{A}_p$ under the single server model, where the computations among the servers are performed in the sequential order. Similarly, the inequality $C_p\le C_1$ is because in the distribute model, servers can send all data to a single server, who then applies $\mathcal{A}_1$ locally. The proportion $C_1/C_p$ measures the degree of balancing the load (\ie, computation cost) of $\mathcal{A}_p$, and we call it \textit{perfect load balanced} if the proportion is $\Theta(p)$. 

\begin{proof}
    First we prove that $n_i=\Theta(n)$ for all $i$ unless with probability $o(2^{-\sigma})$. Note that $n_i$ is the number of elements in the $i$-th server after random shuffle, which follows binomial distribution with parameters $N$ and $1/p$. By Chernoff bound, for any fixed $i\in[p]$, both $\Pr[n_i>2N/p]$ and $\Pr[n_i<N/2p]$ are bounded by $\exp(-\Theta(N/p))=\exp(-\Omega(p\sigma))$. Therefore the probability that $n_i>2N/p$ and $n_i<N/2p$ for any $i\in[p]$ is bounded by  $2\exp(-\Omega(p\sigma)+\log p)=o(2^{-\sigma})$. For the remaining proof we assume $n_i=\Theta(n)$.

    Then we prove that the pivots evenly partition the input to $p$ parts. Formally, let $a_0,a_1,\dots,a_p$ be the pivots taken from the sample. At the final communication step, elements between $a_{i-1}$ and $a_i$ will be sent to the $i$-th server, $i\in[p]$. We are going to prove that each server receives no more than $(1+c_1)n$ elements of the input, where $c_1=o(1)$. Assume the input after sorting is $x_1,\dots,x_N$. If some server receives more than $(1+c_1)n$ elements, then there exists $l\in[N]$ such that $x_l$ is a pivot while any $x_{l+j}$ is not pivot for $0<j\le (1+c_1)n$. This in turn means that $s_l$, the number of sampled elements in $x_{l+1},\dots,x_{l+(1+c_1)n}$, is larger than $n_1/p$, where $n_1$ is the number of elements in the first server after random shuffle, which is also the number of sampled elements. Since $s_l$ follows hypergeometric distribution with parameters $N,n_1,(1+c_1)n$, by Chernoff bound, $\Pr[s_l>n_1/p]$ is at most $\exp(-\Omega(c_1^2 n_1/p))$. By summing $l$ from 1 to $N$, the probability that any server receives more than $(1+c_1)n$ elements is at most $\exp(-\Omega(c_1^2 n_1/p)+\log N)$. Since $n_1=\Theta(n)$ and $n=\omega(p\sigma)$, there exists some $c_1=\Theta(\sqrt{p\sigma/n})=o(1)$ such that the probability is at most $2^{-\sigma-1}$.

    Finally we compute the failure probability of the algorithm by setting padding size $U_i=(1+c_1)(1+c_2)n_i/p$ for $i\in[p]$, given that the pivots have evenly partitioned the input, \ie, in the last round, the total number of elements that should go to the $j$-th server is at most $(1+c_1)n$. The number of elements in the $i$-th server that should go to the $j$-th server, in the worst case, follows the hypergeometric distribution with parameters $N,n_i,(1+c_1)n$, so by Chernoff bound, it is larger than $U_i$ with probability at most $\exp(-\Omega(c_2^2 n_i/p))$. Summing over all $i\in[p]$ and $j\in[p]$, it is bounded by $\exp(-\Omega(c_2^2 n_i/p)+2\log p)$. There exists some $c_2=\Theta\left(\sqrt{p\sigma/n}\right)=o(1)$ such that the probability is at most $2^{-\sigma-1}$. The overall failure probability is therefore bounded by $2^{-\sigma}$ if we set $c=c_1+c_2+c_1c_2=o(1)$.
\end{proof}

A circuit naturally induces an oblivious algorithm under the distributed model, where each level is a round and each gate with two inputs from different servers requires a communication. Therefore, the number of rounds of the algorithm is equal to the depth of the circuit. However, existing circuits for database joins are all with at least $O(\log^2 N)$ depth~\cite{10.1145/3517804.3524142,10.14778/3407790.3407814} and hence induce algorithms with polylogarithm number of rounds. This has no advantage to all algorithms mentioned above, which are in constant number of rounds.
